A comparison between short GRB afterglows and AT2017gfo: shedding light on kilonovae properties

Multi-messenger astronomy received a great boost following the discovery of kilonova AT2017gfo, the optical counterpart of the gravitational wave source GW170817 associated with the short gamma-ray burst GRB 170817A. AT2017gfo was the first kilonova that could be extensively monitored in time both photometrically and spectroscopically. Previously, only few candidates have been observed against the glare of short GRB afterglows. In this work, we aim to search the fingerprints of AT2017gfo-like kilonova emissions in the optical/NIR light curves of 39 short GRBs with known redshift. For the first time, our results allow us to study separately the range of luminosity of the blue and red components of AT2017gfo-like kilonovae in short GRBs. In particular, the red component is similar in luminosity to AT2017gfo, while the blue kilonova can be more than 10 times brighter. Finally, we find further evidence to support all the claimed kilonova detections and we exclude an AT2017gfo-like kilonova in GRBs 050509B and 061201.

==> README <==
% readme.txt
%
% MNRAS journal LaTeX package
% v3.0 for LaTeX 2e
%
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `author-maintained'.
% 
% The Current Maintainer of this work is: Royal Astronomical Society,
% MNRAS Editorial Office, who can be contacted on mn@ras.org.uk
%
% This work consists of all the files listed in readme.txt
%
%
% Last updated 22 May 2015
%
% Copyright (C) Royal Astronomical Society 2015, Blackwell Science 2001,
% Cambridge University Press 1994
%
% See each file for a detailed author list and change log.
%
% This package consists of the following files:

readme.txt          This file

mnras.cls           MNRAS LaTeX document class
mnras.bst           MNRAS BibTeX style

mnras_guide.tex     User guide, LaTeX format
mnras_guide.pdf     User guide, PDF format
mnras_template.tex  A simple template paper

example.eps         An example image used in the guide
example.png         An example image used in the guide
example.ps          An example image used in the guide

legacy\legacy.txt   Description of the legacy releases
legacy\mn2e.cls     v2.2 of mn2e.cls (deprecated)
legacy\mn2e.bst     v1.1b of mn2e.bst (deprecated)


% Disclaimer:
%
% This LaTeX package is provided free to the community in the hope that it
% assists them in preparing papers for the journal Monthly Notices of the
% Royal Astronomical Society.
% The files are provided 'as-is' with no guarantee of their suitability,
% freedom from errors or omissions, or compatibility with any software.
% The Royal Astronomical Society cannot provide user support for this package,
% LaTeX, or for any other software.
% Authors are free to use other styles or programmes if they wish.
% Please see the journal instructions to authors for guidance.
% This disclaimer is in addition to the No Warranty section of the licence,
% at the link given above.

==> legacy/tab1short.tex <==
%\clearpage
\onecolumn


%\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
%\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}

%\begin{table*}
%\begin{longtable}{l c c c c c c c }
%\begin{longtable}{l p{1cm} p{3.5cm} p{0.8cm}p{1.5cm}p{1.7cm}p{1.5cm} p{3cm}}
\begin{longtable}{l p{1cm} p{3.5cm} p{0.8cm}p{1.6cm}p{1.85cm}p{1.3cm} p{3.1cm}}
%\begin{tabular}{c@{\hspace{10cm}}c}
%\renewcommand{\setlength{\tabcolsep}}{2pt}
\caption{Short GRBs with known redshift in addition to the \citet{Fong2015a} sample }\label{tab:newgrbs}\\
GRB & $\Delta T$ & Telescope/Instr & Filter & mag & Flux density & Gal. Ext. & Refs\\
    &  hours &   &   &   & $\mu Jy$ & A$_V$ & \\ 
 \hline
 \hline
\endfirsthead

\multicolumn{8}{c}{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\ \midrule
\endhead

\midrule \multicolumn{8}{|r|}{{Continued on next page}} \\ \midrule
\endfoot

\midrule 
\endlastfoot

\toprule  

%\small
%\tiny
\footnotetext
%\large
  
 130603B	  	&	700	&	  HST  	&	  F160W  	&	$>$  26.90	   &	$<$ 0.065	&	0.06	&	\citet{Tanvir2013a}  \\
160410A	  	&	0.533	&	  ESO/MPG GROND  	&	  g	&	  20.60$\pm$ 0.10	 	&    21.89$\pm$ 2.112    	&	0.02	&	  GCN\#19272  \\
  	&	0.533	&	    ESO/MPG GROND   	&	       r     	&	     20.50$\pm$ 0.10  	&	  23.86$\pm$ 2.302  	&		&	   \\
  	&	 	  0.533	 	&	    ESO/MPG GROND   	&	  	i      	&	   20.70$\pm$ 0.10  	&	  19.76$\pm$1.907  	&		&	      \\
  	&	 	  0.533	 	&	    ESO/MPG GROND   	&	  	z     	&	  	 20.50$\pm$ 0.20  	&	   23.67$\pm$4.788  	&		&	     \\
